Shannon Entropy Estimation in $\infty$-Alphabets from Convergence Results

The problem of Shannon entropy estimation in countable infinite alphabets is addressed from the study and use of convergence results of the entropy functional, which is known to be discontinuous with respect to the total variation distance in $\infty$-alphabets. Sufficient conditions for the convergence of the entropy are used, including scenarios with both finitely and infinitely supported assumptions on the distributions. From this new perspective, four plug-in histogram-based estimators are studied showing that convergence results are instrumental to derive new strong consistency and rate of convergences results. Different scenarios and conditions are used on both the estimators and the underlying distribution, considering for example finite and unknown supported assumptions and summable tail bounded conditions.

==> main_jorge_silva <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Jorge Silva at 2017-04-04 16:53:08 -0300 


%% Saved with string encoding Unicode (UTF-8) 



@inproceedings{valiant_2010,
	Author = {G. Valiant and P. Valiant},
	Booktitle = {Proc. Electrom. Colloq. Comput. Complex.},
	Date-Added = {2017-03-02 14:48:28 +0000},
	Date-Modified = {2017-03-02 14:51:00 +0000},
	Pages = {179},
	Title = {A {CLT} and tight lower bounds for estimating entropy},
	Volume = {17},
	Year = {2010}}

@inproceedings{valiant_2011,
	Author = {G. Valiant and P. Valiant},
	Booktitle = {in Proc. 43rd Annu. ACM Symp. Theory Comput.},
	Date-Added = {2017-03-02 14:43:35 +0000},
	Date-Modified = {2017-03-02 14:46:44 +0000},
	Pages = {685-694},
	Title = {Estimating the unseen: An $n/log(n)$-sample estimator for entropy and support size, shown opitmal via new CLTs},
	Year = {2011}}

@book{tsybakov_2009,
	Author = {A. B. Tsybakov},
	Date-Added = {2017-03-01 18:10:11 +0000},
	Date-Modified = {2017-03-01 18:23:28 +0000},
	Publisher = {New York: Springer-Verlag},
	Title = {Introduction to non-parametric estimation},
	Year = {2009}}

@article{jiao_2015,
	Author = {J. Jiao and K. Venkat and Y. Han and T. Weissman},
	Date-Added = {2017-02-27 14:30:54 +0000},
	Date-Modified = {2017-02-27 14:33:02 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Title = {Minimax Estimation of Functionals of Discrete Distributions},
	Volume = {61},
	Year = {2015}}

@article{wu_2016,
	Author = {Y. Wu and P. Yang},
	Date-Added = {2017-02-27 13:57:42 +0000},
	Date-Modified = {2017-03-11 02:34:27 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Title = {MInimax Rates of Entropy Estimation on Large Alphabets via best Plynomial Approximation},
	Volume = {62},
	Year = {2016}}

@book{vaart_2000,
	Author = {A. W. {Van der Vaart}},
	Date-Added = {2017-02-27 13:35:21 +0000},
	Date-Modified = {2017-02-27 13:36:46 +0000},
	Publisher = {Cambridge Univ Press},
	Title = {Asymtotic Statistics},
	Volume = {3},
	Year = {2000}}

@article{paniski_2003,
	Author = {Liam Paninski},
	Date-Added = {2016-12-01 19:20:46 +0000},
	Date-Modified = {2016-12-01 19:20:46 +0000},
	Journal = {Neural Computation},
	Number = {6},
	Pages = {1191-1254},
	Title = {Estimation of Entropy and Mutual Information},
	Volume = {15},
	Year = {2003}}

@article{paniski_2004,
	Author = {L. Paninski},
	Date-Added = {2016-12-01 19:20:37 +0000},
	Date-Modified = {2017-03-11 02:30:59 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Number = {9},
	Pages = {2200-2203},
	Title = {Estimating entropy on m bins given fewer than m samples},
	Volume = {50},
	Year = {2004}}

@conference{silva_isit_2012,
	Author = {J.F. Silva and P. Parada},
	Booktitle = {International Symposium on Information Theory},
	Date-Added = {2016-12-01 19:08:56 +0000},
	Date-Modified = {2017-04-04 19:52:36 +0000},
	Month = {June},
	Organization = {IEEE},
	Title = {Shannon Entropy Convergence Results in the Countable Infinite Case},
	Year = {2012}}

@book{yeung_2002,
	Author = {Raymond W. Yeung},
	Date-Added = {2013-07-28 19:22:53 +0000},
	Date-Modified = {2013-07-28 19:25:55 +0000},
	Publisher = {Kluwer Academic / Plenum Publisher, New York},
	Title = {A first Course on Information Theory},
	Year = {2002}}

@article{wehrl_1978,
	Author = {A. Wehrl},
	Date-Added = {2013-07-08 14:21:15 +0000},
	Date-Modified = {2013-07-08 14:22:23 +0000},
	Journal = {Rev. Mod. Phys.},
	Pages = {221-260},
	Title = {General Properties of entropy},
	Volume = {50},
	Year = {1978}}

@article{kemperman_1969,
	Author = {J. Kemperman},
	Date-Added = {2013-07-01 14:23:12 +0000},
	Date-Modified = {2013-07-01 14:24:44 +0000},
	Journal = {Ann. Math. Statist.},
	Month = {December},
	Pages = {2156-2177},
	Title = {On the optimum rate of transmitting information},
	Volume = {40},
	Year = {1969}}

@article{silva_2012_jspi,
	Author = {Jorge F Silva and Patricio Parada},
	Date-Added = {2013-06-24 14:12:27 +0000},
	Date-Modified = {2013-06-28 14:48:30 +0000},
	Journal = {Journal of Statistical Planning and Inference},
	Number = {7},
	Pages = {1716-1732},
	Title = {On the Convergence of {S}hannon Differential Entropy, and its Connections with Density and Entropy Estimation},
	Volume = {142},
	Year = {2012}}

@article{silva_2012,
	Author = {J.F. Silva and S.N. Narayanan},
	Date-Added = {2013-04-08 16:19:59 +0000},
	Date-Modified = {2017-03-11 02:32:57 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Month = {March},
	Number = {3},
	Pages = {940 -- 1952},
	Read = {1},
	Title = {Complexity-Regularized Tree-Structured Partition for Mutual Information Estimation},
	Volume = {58},
	Year = {2012}}

@article{antos_2002,
	Author = {A. Antos and I. Kontoyiannis},
	Date-Added = {2013-03-26 14:42:03 +0000},
	Date-Modified = {2013-03-26 14:48:37 +0000},
	Journal = {Random Structures and Algorithms},
	Month = {October-December},
	Number = {3-4},
	Pages = {163-193},
	Title = {Convergence Properties of fucntionals estimates for discrete distributions},
	Volume = {19},
	Year = {2001}}

@article{boucheron_2009,
	Author = {S. Boucheron and A. Gariver and E. Gassiat},
	Date-Added = {2012-02-02 15:52:32 -0300},
	Date-Modified = {2012-02-02 15:52:32 -0300},
	Journal = {IEEE Transactions on Information Theory},
	Month = {January},
	Number = {1},
	Pages = {358-373},
	Rating = {4},
	Read = {1},
	Title = {Coding on Countable Infinite Alphabets},
	Volume = {55},
	Year = {2009}}

@book{rissanen_2010,
	Author = {Jorma Rissanen},
	Date-Added = {2011-09-23 16:35:26 -0300},
	Date-Modified = {2011-09-23 16:37:21 -0300},
	Publisher = {Sprimger},
	Rating = {4},
	Title = {Information and Complexity in Statistical Modeling},
	Year = {2010}}

@book{cover_2006,
	Author = {T. M. Cover and J. A. Thomas},
	Date-Added = {2011-09-23 16:32:16 -0300},
	Date-Modified = {2011-09-23 16:33:09 -0300},
	Edition = {2do},
	Publisher = {Wiley Interscience, New York},
	Title = {Elements of Information Theory},
	Year = {2006}}

@article{ho_2010b,
	Author = {Siu-Wai Ho and Raymond W. Yeung},
	Date-Added = {2011-08-23 16:51:28 -0300},
	Date-Modified = {2011-08-23 16:52:50 -0300},
	Journal = {IEEE Transactions on Information Theory},
	Month = {December},
	Number = {12},
	Pages = {5893-5905},
	Rating = {3},
	Read = {1},
	Title = {On information divegence measures and Unified typicality},
	Volume = {56},
	Year = {2010}}

@book{ash_1965,
	Author = {Robert B. Ash},
	Date-Added = {2011-08-23 16:44:06 -0300},
	Date-Modified = {2011-08-23 16:45:08 -0300},
	Publisher = {Dover Publications},
	Title = {Information Theory},
	Year = {1965}}

@article{gyorfi_1994b,
	Author = {L. Gy{\"o}rfi and I. P\'{a}li and E. C. {van der Meulen}},
	Date-Added = {2011-07-21 13:45:30 -0400},
	Date-Modified = {2017-03-11 02:38:31 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Number = {1},
	Pages = {267-271},
	Rating = {4},
	Read = {1},
	Title = {There is no Universal Source Code for an Infinity Source ALphabet},
	Volume = {40},
	Year = {1994}}

@inbook{harremoes_2007,
	Author = {P. Herremo\"{e}s},
	Chapter = {Information topologies with applications},
	Date-Added = {2011-07-08 11:48:08 -0400},
	Date-Modified = {2013-06-28 14:52:27 +0000},
	Editor = {I. Csisz\'{a}r and G. KAtona and G. Tardos},
	Pages = {113-150},
	Publisher = {Sprimger},
	Series = {Bolyai Society of Mathematical Studies},
	Title = {Entropy. Search, Complexity},
	Volume = {16},
	Year = {2007}}

@article{ho_2010,
	Author = {S.-W. Ho and R. W. Yeung},
	Date-Added = {2011-07-08 11:46:12 -0400},
	Date-Modified = {2017-03-11 02:30:04 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Month = {December},
	Number = {12},
	Pages = {5906-5929},
	Title = {The Interplay between Entropy and Variational Distance},
	Volume = {56},
	Year = {2010}}

@article{rissanen_1984,
	Author = {J. Rissanen},
	Date-Added = {2011-03-23 14:25:05 -0400},
	Date-Modified = {2011-03-23 14:26:45 -0400},
	Journal = {IEEE Transactions on Information Theory{\c c}},
	Month = {July},
	Number = {4},
	Pages = {629-636},
	Title = {Universal Coding, information, prediction, and estimation},
	Volume = {IT-30},
	Year = {1984}}

@article{linder_1994,
	Author = {T. Linder and Gabor Lugosi and K. Zeger},
	Date-Added = {2011-03-23 13:25:52 -0400},
	Date-Modified = {2011-03-23 13:28:00 -0400},
	Journal = {IEEE Transactions on Information Theory},
	Month = {November},
	Number = {6},
	Pages = {1728-1740},
	Title = {Rates of convergence in the source codign theorem, in empirical quantization design, and in univesal lossy source codign},
	Volume = {40},
	Year = {1994}}

@article{lider_1995,
	Author = {T. Linder and Gabor Lugosi and K. Zeger},
	Date-Added = {2011-03-23 13:23:01 -0400},
	Date-Modified = {2011-03-23 13:25:19 -0400},
	Journal = {IEEE Transactions on Information Theory},
	Month = {May},
	Number = {6},
	Pages = {665-676},
	Title = {Fixed-rate universal lossy soruce codign and rate of convergence for memoryless sources},
	Volume = {41},
	Year = {1995}}

@article{neuhoff_1975,
	Author = {D. L. Neuhoff and Robert M. Gray and Lee D. Davisson},
	Date-Added = {2011-03-23 13:20:22 -0400},
	Date-Modified = {2011-03-23 13:22:24 -0400},
	Journal = {IEEE Transactions on Information Theory},
	Month = {September},
	Number = {5},
	Pages = {511-523},
	Title = {Fixed rate universal block source coding with a fidelity criterion},
	Volume = {IT-21},
	Year = {1975}}

@article{chou_1996,
	Author = {P. Chou and M. Effros and Robert M. Gray},
	Date-Added = {2011-03-23 13:16:51 -0400},
	Date-Modified = {2011-03-23 13:19:14 -0400},
	Journal = {IEEE Transactions on Information Theory},
	Month = {July},
	Number = {4},
	Pages = {1109-1138},
	Title = {A vector quantization approach to universal noiseless coding and quantization},
	Volume = {42},
	Year = {1996}}

@inbook{devroye_2001b,
	Author = {L. Devroye and L. Gy{\"o}rfi},
	Chapter = {Distribution and Density Estimation},
	Date-Added = {2011-03-08 16:58:39 -0300},
	Date-Modified = {2011-03-08 17:02:19 -0300},
	Editor = {L. Gy{\"o}rfi},
	Publisher = {Springer - Verlag, New York},
	Title = {Principles of Nonparametric Learning},
	Year = {2001}}

@article{raginsky_2008,
	Author = {Maxim Raginsky},
	Date-Added = {2011-01-04 10:57:54 -0300},
	Date-Modified = {2011-01-04 10:59:39 -0300},
	Journal = {IEEE Transactions on Information Theory},
	Number = {7},
	Pages = {3059-3077},
	Rating = {4},
	Read = {1},
	Title = {Joint Fixed-Rate Univesal Lossy Coding and Identification of Continuous-Alphabet Memoryless Sources},
	Volume = {54},
	Year = {2008}}

@article{yatracos_1988,
	Author = {Y. G. Yatracos},
	Date-Added = {2010-12-28 11:32:05 -0300},
	Date-Modified = {2010-12-28 11:34:30 -0300},
	Journal = {The Canadian Jounal of Statistics},
	Number = {3},
	Pages = {283-292},
	Rating = {5},
	Read = {1},
	Title = {A note on $L_1$ consistent estimation},
	Volume = {16},
	Year = {1988}}

@article{dudley_1978,
	Author = {R. M. Dudley},
	Date-Added = {2010-12-27 11:55:16 -0300},
	Date-Modified = {2010-12-27 11:56:45 -0300},
	Journal = {Annals of Probability},
	Pages = {899-929},
	Title = {Central Limits Theorems for Empirical Measures},
	Volume = {6},
	Year = {1978}}

@article{devroye_1997,
	Author = {L. Devroye and G. Lugosi},
	Date-Added = {2010-12-22 11:15:41 -0300},
	Date-Modified = {2010-12-22 11:17:06 -0300},
	Journal = {Annals of Statistics},
	Number = {2626-2637},
	Title = {Nonasymtotic universal smothing factors, kernel complexity and Yatracos classes},
	Volume = {25},
	Year = {1997}}

@article{devroye_1996,
	Author = {L. Devroye and G. Lugosi},
	Date-Added = {2010-12-22 11:10:40 -0300},
	Date-Modified = {2010-12-22 11:13:12 -0300},
	Journal = {Annals of Statistics},
	Number = {2499-2512},
	Title = {A universally acceptable smoothing factor for kernel density estimation},
	Volume = {24},
	Year = {1996}}

@article{yatracos_1985,
	Author = {Y. G. Yatracos},
	Date-Added = {2010-12-21 15:48:59 -0300},
	Date-Modified = {2010-12-21 15:50:33 -0300},
	Journal = {The Annals of Statistics},
	Number = {2},
	Pages = {768-774},
	Title = {Rates of Convergence of Minimum Distance Estimators and {K}olmogorov`s Entropy},
	Volume = {13},
	Year = {1885}}

@article{kolmogorov_1961,
	Author = {A. N. Kolmogorov and V. M. Tikhomirov},
	Date-Added = {2010-12-21 15:39:21 -0300},
	Date-Modified = {2010-12-21 15:39:21 -0300},
	Journal = {Translation of the American Mathematical Society},
	Pages = {277-364},
	Title = {$\epsilon$-emtropy and $\epsilon$-capacity of sets in function spaces},
	Volume = {17},
	Year = {1961}}

@article{ho_2009,
	Author = {S.-W. Ho and R. W. Yeung},
	Date-Added = {2010-10-27 15:41:07 -0300},
	Date-Modified = {2017-03-11 02:29:28 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Month = {December},
	Number = {12},
	Pages = {5362-5374},
	Title = {On the discontinuity of the {S}hannon Information Measures},
	Volume = {55},
	Year = {2009}}

@article{vajda_2001,
	Author = {I. Vajda and E. C. {van der Meulen}},
	Date-Added = {2010-10-26 08:03:34 -0300},
	Date-Modified = {2017-03-11 02:34:00 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Month = {July},
	Number = {5},
	Pages = {1867-1883},
	Title = {Optimization of {B}arron Density Estimates},
	Volume = {47},
	Year = {2001}}

@article{abou-jaoude-1976b,
	Author = {S. Abou-Jaoude},
	Date-Added = {2010-09-07 18:06:53 -0400},
	Date-Modified = {2010-09-07 18:07:39 -0400},
	Journal = {Ann. Inst. H. Poincar\'{e}},
	Pages = {213-231},
	Title = {Condition n\'{e}cessaires et sufficantes de convergence ${L}_1$ en probabilit\'{e} de l`hitograme pour une densit\'{e}},
	Volume = {12},
	Year = {1976}}

@article{silva_2010b,
	Author = {J.F. Silva and S.N. Narayanan},
	Date-Added = {2010-09-03 13:11:23 -0400},
	Date-Modified = {2017-04-04 19:53:07 +0000},
	Journal = {Journal of Statistical Planning and Inference},
	Month = {November},
	Number = {11},
	Pages = {3180 - 3198},
	Read = {1},
	Title = {Information divergence estimation based on data-dependent partitions},
	Volume = {140},
	Year = {2010}}

@article{silva_2010,
	Author = {J.F. Silva and S. N. Narayanan},
	Date-Added = {2010-09-01 12:34:07 -0400},
	Date-Modified = {2017-03-11 02:32:07 +0000},
	Journal = {IEEE Transactions on Signal Processing},
	Month = {July},
	Number = {7},
	Pages = {3497-3511},
	Read = {1},
	Title = {Non-Product Data-Dependent Partitions for Mutual Information Estimation: Strong Consistency and Applications},
	Volume = {58},
	Year = {2010}}

@article{kullback_1951,
	Author = {S. Kullback and R. Leibler},
	Date-Added = {2010-08-17 10:35:25 -0400},
	Date-Modified = {2010-08-17 10:37:13 -0400},
	Journal = {Ann. Math. Statist.},
	Pages = {79-86},
	Title = {On Information and Sufficiency},
	Volume = {22},
	Year = {1951}}

@book{billingsley_1999,
	Author = {P. Billingsley},
	Date-Added = {2010-08-11 11:59:26 -0400},
	Date-Modified = {2010-08-11 12:02:19 -0400},
	Edition = {second edition},
	Publisher = {Wiley Series in Probability and Statistics},
	Title = {Convergence of Probability Measures},
	Year = {1999}}

@article{kullback_1967,
	Author = {S. Kullback},
	Date-Added = {2010-08-06 14:55:37 -0400},
	Date-Modified = {2013-07-24 22:09:03 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Pages = {126-127},
	Title = {A lower bound for discrimination in terms of variation},
	Volume = {13},
	Year = {1967}}

@article{scheffe_1947,
	Author = {H. Scheff\'{e}},
	Date-Added = {2010-08-06 14:00:18 -0400},
	Date-Modified = {2010-12-22 10:56:06 -0300},
	Journal = {Ann. Math. Statist.},
	Pages = {434-458},
	Title = {A Useful convergence theorem for probability distribution},
	Volume = {18},
	Year = {1947}}

@article{berlinet_2001,
	Author = {J. Beirlant and L. Devroye and L. Gy{\"o}rfi and Igor Vajda},
	Date-Added = {2010-03-19 10:56:12 -0400},
	Date-Modified = {2010-03-19 10:57:59 -0400},
	Journal = {Journal of Statistical Planing and Inference},
	Pages = {1-16},
	Rating = {4},
	Title = {Large deviation of divergence measures on partitions},
	Volume = {93},
	Year = {2001}}

@book{csiszar_2004,
	Author = {I. Csisz\'{a}r and P. C. Shields},
	Date-Added = {2010-03-19 08:36:11 -0400},
	Date-Modified = {2017-03-11 02:37:48 +0000},
	Publisher = {Now Inc.},
	Title = {Information theory and Statistics: A tutorial},
	Year = {2004}}

@article{berlinet_2005,
	Author = {A. Berlinet and Igor Vajda},
	Date-Added = {2010-03-15 10:29:35 -0400},
	Date-Modified = {2010-03-15 10:31:37 -0400},
	Journal = {Journal of Statistical Planing and Inference},
	Keywords = {asymptotically sufficient partitions},
	Pages = {4217-4238},
	Rating = {5},
	Read = {1},
	Title = {On asymtotic sufficiency and optimality of quantizations},
	Volume = {136},
	Year = {2005}}

@book{liese_1987,
	Date-Added = {2010-03-15 09:54:35 -0400},
	Date-Modified = {2010-03-15 09:55:08 -0400},
	Title = {Convex}}

@article{silva_2009,
	Author = {Jorge Silva and Shrikanth Narayanan},
	Date-Added = {2009-08-14 13:53:00 -0400},
	Date-Modified = {2010-03-15 17:57:22 -0400},
	Journal = {IEEE Transactions on Signal Processing},
	Number = {5},
	Pages = {1796-1810},
	Read = {Yes},
	Title = {Discriminative Wavelet Packet Filter Bank Selection for Pattern Recognition},
	Volume = {57},
	Year = {2009}}

@inproceedings{gyorfi_1994,
	Author = {L. Gy{\"o}rfi and Edward C. {Van der Meulen}},
	Booktitle = {IEEE International Symposium on Information Theory},
	Date-Added = {2009-07-10 09:44:49 -0400},
	Date-Modified = {2010-11-15 16:48:51 -0300},
	Pages = {35-35},
	Title = {Density Estimation Consistent in Information Divergence},
	Year = {1994}}

@article{wang_2009,
	Author = {Q. Wang and Sanjeev R. Kulkarni and Sergio Verd\'{u}},
	Date-Added = {2009-07-09 18:43:03 -0400},
	Date-Modified = {2010-03-15 17:58:19 -0400},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Pages = {2392-2405},
	Title = {Divergence Estimation for Multidimensional Densities via K-Nearest-Neighbor Distance},
	Volume = {55},
	Year = {2009}}

@article{paninski_2008,
	Author = {L. Paninski},
	Date-Added = {2009-07-09 17:38:30 -0400},
	Date-Modified = {2009-07-09 17:39:57 -0400},
	Journal = {IEEE Transactions on Information Theory},
	Number = {9},
	Pages = {4384-4388},
	Title = {Undersmoothed Kernel Entropy Estimation},
	Volume = {54},
	Year = {2008}}

@article{paninski_2003,
	Author = {L. Paninski},
	Date-Added = {2009-07-09 17:35:59 -0400},
	Date-Modified = {2009-07-09 17:37:47 -0400},
	Journal = {Neural Comput.},
	Pages = {1191-1253},
	Title = {Estimation of Entropy and Mutual Information},
	Volume = {15},
	Year = {2003}}

@article{beirlant_1997,
	Author = {J. Beirlant and E. Dudewicz and L. Gy{\"o}rfi and E. C. {van der Meulen}},
	Date-Added = {2009-07-09 17:31:49 -0400},
	Date-Modified = {2017-03-11 02:36:31 +0000},
	Journal = {Int. Math. Statist. Sci.},
	Pages = {17-39},
	Title = {Nonparametric entropy Estimation: An Overview},
	Volume = {6},
	Year = {1997}}

@conference{silva_isit_2007,
	Author = {J. Silva and S. Narayanan},
	Booktitle = {IEEE International Symposium on Information Theory},
	Date-Added = {2009-01-21 10:32:36 -0300},
	Date-Modified = {2009-01-21 10:33:19 -0300},
	Organization = {IEEE},
	Read = {Yes},
	Title = {Universal Consistency of Data-Driven Partitions for Divergence Estimation},
	Year = {2007}}

@article{piera_2009,
	Author = {F. Piera and P. Parada},
	Date-Added = {2009-01-20 16:25:18 -0300},
	Date-Modified = {2017-03-11 02:31:19 +0000},
	Journal = {Problems of Information Transmission},
	Number = {2},
	Pages = {75-94},
	Rating = {4},
	Read = {Yes},
	Title = {On Convergence Properties of {S}hannon Entropy},
	Volume = {45},
	Year = {2009}}

@article{berlinet_1998,
	Author = {A. Berlinet and I. Vajda and E. C. {van der Meulen}},
	Date-Added = {2008-11-19 18:18:42 -0800},
	Date-Modified = {2017-03-11 02:36:57 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Number = {3},
	Pages = {999-1009},
	Rating = {1},
	Read = {No},
	Title = {About the asymptotic accuracy of {B}arron density estimate},
	Volume = {44},
	Year = {1998}}

@article{gyorfi_1998,
	Author = {L. Gy{\"o}rfi and F. Liese and Igor Vajda and Edward C. {Van der Meulen}},
	Date-Added = {2008-11-19 18:13:48 -0800},
	Date-Modified = {2010-11-15 16:49:53 -0300},
	Journal = {Statistics},
	Number = {1},
	Pages = {31-57},
	Title = {Distribution Estimates consistent in $\chi^2$- divergence},
	Volume = {32},
	Year = {1998}}

@article{gyorfi_1987,
	Author = {L. Gy{\"o}rfi and Edward C. {van der Meulen}},
	Date-Added = {2008-11-19 18:08:12 -0800},
	Date-Modified = {2013-06-20 14:58:02 +0000},
	Journal = {Computational Statistics and Data analysis},
	Pages = {425-426},
	Rating = {4},
	Read = {Yes},
	Title = {Density-free convergence properties of various estimators of entropy},
	Volume = {5},
	Year = {1987}}

@book{devroye_1985,
	Author = {L. Devroye and L. Gy{\"o}rfi},
	Date-Added = {2008-11-19 18:04:59 -0800},
	Date-Modified = {2010-03-15 10:47:48 -0400},
	Publisher = {Wiley Interscience, New York},
	Title = {Nonparametric density estimation: The $L_1$ view},
	Year = {1985}}

@book{liese_vajda_1987,
	Author = {F. Liese and Igor Vajda},
	Date-Added = {2008-11-15 10:44:46 -0800},
	Date-Modified = {2010-03-15 10:32:05 -0400},
	Keywords = {asymptotically sufficient partitions},
	Publisher = {Teubner-Verlag, Germany},
	Title = {Convex Statistical Distances},
	Year = {1987}}

@article{barron_1992,
	Author = {A. Barron and L. Gy{\"o}rfi and E. C. {van der Meulen}},
	Date-Added = {2008-11-01 12:52:32 -0700},
	Date-Modified = {2017-03-11 02:30:30 +0000},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Pages = {1437-1454},
	Rating = {4},
	Read = {Yes},
	Title = {Distribution Estimation Consistent in Total Variation and in Two Types of Information Divergence},
	Volume = {38},
	Year = {1992}}

@article{csiszar_1967,
	Author = {I. Csisz\'{a}r},
	Date-Added = {2008-10-25 15:30:39 -0700},
	Date-Modified = {2008-10-25 15:33:20 -0700},
	Journal = {Studia Scient. Mathe. Hung.},
	Pages = {299-318},
	Title = {Information-type measures of difference of probability distributions and indirect observations},
	Volume = {2},
	Year = {1967}}

@conference{csiszar_1973,
	Author = {I. Csisz\'{a}r},
	Booktitle = {Trans. 6th Prague Confe. Information Theory, Statistical Decision Functions, and Random Processes},
	Date-Added = {2008-10-25 13:06:15 -0700},
	Date-Modified = {2008-10-25 13:10:39 -0700},
	Editor = {Academia},
	Pages = {159-174},
	Title = {Generalized Entropy and Quantization Problems},
	Year = {1973}}

@article{vajda_2002,
	Author = {Igor Vajda},
	Date-Added = {2008-10-25 13:02:38 -0700},
	Date-Modified = {2010-03-15 17:57:38 -0400},
	Journal = {IEEE Transactions on Information Theory},
	Keywords = {asymptotically sufficient partitions},
	Number = {8},
	Pages = {2163-2172},
	Rating = {3},
	Read = {Yes},
	Title = {On Convergence of Information Contained in Quantized Observations},
	Volume = {48},
	Year = {2002}}

@article{poor_1977,
	Author = {H. V. Poor and J. B. Tomas},
	Date-Added = {2007-12-03 19:06:45 -0800},
	Date-Modified = {2010-03-15 17:56:55 -0400},
	Journal = {IEEE Trans. on Comm.},
	Number = {9},
	Pages = {893-900},
	Title = {Applications of {A}li-{S}ilvey Distance Measures in the Design Generalized Quantizers for Binary Decision Systems},
	Volume = {25},
	Year = {1977}}

@article{jain_2002,
	Author = {Avinash Jain and Pierre Moulin and Michael Miller and Kannan Ramchandran},
	Date-Added = {2007-12-03 14:40:40 -0800},
	Date-Modified = {2010-03-15 17:55:55 -0400},
	Journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Number = {9},
	Pages = {1153-1166},
	Read = {Yes},
	Title = {Information-Theoretic Bounds on Target Recognition Performance Based on Degraded Image Data},
	Volume = {24},
	Year = {2002}}

@article{liese_2006,
	Author = {F. Liese and Domingo Morales and Igor Vajda},
	Date-Added = {2007-11-21 10:10:48 -0800},
	Date-Modified = {2010-03-15 10:32:00 -0400},
	Journal = {IEEE Transactions on Information Theory},
	Keywords = {asymptotically sufficient partitions},
	Number = {12},
	Pages = {5599-5606},
	Rating = {3},
	Read = {Yes},
	Title = {Asymptotically Sufficient Partition and Quantization},
	Volume = {52},
	Year = {2006}}

@article{vasconcelos2004_b,
	Author = {Nuno Vasconcelos},
	Date-Added = {2007-07-23 17:23:06 -0700},
	Date-Modified = {2007-07-23 17:24:18 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {7},
	Pages = {1482-1496},
	Rating = {4},
	Read = {Yes},
	Title = {On the Efficient Evaluation of Probabilistic Similarity Functions for Image Retrieval},
	Volume = {50},
	Year = {2004}}

@article{juang85,
	Author = {B. H. Juang and L. R. Rabiner},
	Date-Added = {2007-07-23 17:20:57 -0700},
	Date-Modified = {2010-03-15 18:01:47 -0400},
	Journal = {AT\&T Technical Journal},
	Number = {2},
	Pages = {391-408},
	Rating = {3},
	Read = {Yes},
	Title = {A probabilistic distance measure for hidden {M}arkov models},
	Volume = {64},
	Year = {1985}}

@conference{singer96,
	Author = {Y. Singer and M.K. Warmuth},
	Booktitle = {Advances in Neural Information Processing System 9},
	Date-Added = {2007-07-23 17:18:12 -0700},
	Date-Modified = {2010-03-15 18:02:09 -0400},
	Publisher = {Morgan Kaufmann Publishers},
	Read = {Yes},
	Title = {Training Algorithm for Hidden {M}arkov Models Using Entropy Based Distance Functions},
	Year = {1996}}

@conference{nguyen_isit_2007,
	Author = {Xuan{L}ong Nguyen and Martin Wainwright and Michael Jordan},
	Booktitle = {IEEE International Symposium on Information Theory},
	Date-Added = {2007-07-23 17:04:32 -0700},
	Date-Modified = {2010-03-15 17:56:11 -0400},
	Organization = {IEEE},
	Rating = {4},
	Read = {Yes},
	Title = {Nonparametric estimation of the likelihood ratio and divergence functionals},
	Year = {2007}}

@inproceedings{silva_mlsp_2007,
	Author = {Jorge Silva and Shrikanth Narayanan},
	Booktitle = {IEEE Workshop Machine Learning for Signal Processing},
	Date-Added = {2007-07-21 21:09:28 -0700},
	Date-Modified = {2007-07-21 21:12:33 -0700},
	Month = {August},
	Rating = {3},
	Read = {Yes},
	Title = {Minimum Probability of Error Signal Representation},
	Year = {2007}}

@article{cover_1965,
	Author = {T. M. Cover},
	Date-Added = {2007-05-15 15:11:08 -0700},
	Date-Modified = {2007-05-15 15:13:55 -0700},
	Journal = {IEEE Trans. on Electronic Computers},
	Pages = {326-334},
	Title = {Geometrical and Statistical Properties of Systems of Linear Inequalities with Applications in Pattern Recognition},
	Volume = {14},
	Year = {1965}}

@article{nobel_1996b,
	Author = {Andrew B. Nobel},
	Date-Added = {2007-05-11 17:36:35 -0700},
	Date-Modified = {2007-05-11 17:38:05 -0700},
	Journal = {The Annals of Statistics},
	Number = {3},
	Pages = {1084-1105},
	Title = {Histogram Regression Estimation Using Data-Dependent Partitions},
	Volume = {24},
	Year = {1996}}

@book{hollander_2000,
	Author = {Frank den Hollander},
	Date-Added = {2007-02-22 20:37:41 -0800},
	Date-Modified = {2007-02-22 20:38:55 -0800},
	Publisher = {American Mathematical Society},
	Rating = {5},
	Read = {Yes},
	Title = {Large Deviations},
	Year = {2000}}

@book{devroye_2001,
	Author = {L. Devroye and G. Lugosi},
	Date-Added = {2007-01-02 10:26:22 -0800},
	Date-Modified = {2007-01-02 10:28:18 -0800},
	Publisher = {Springer - Verlag, New York},
	Title = {Combinatorial Methods in Density Estimation},
	Year = {2001}}

@article{gessaman_1970,
	Author = {M. P. Gessaman},
	Date-Added = {2006-12-30 12:30:24 -0800},
	Date-Modified = {2006-12-30 12:31:11 -0800},
	Journal = {Ann. Math. Statist.},
	Pages = {1344-1346},
	Title = {A consistent nonparametric multivariate density estimator based on statistically equivalent blocks},
	Volume = {41},
	Year = {1970}}

@article{wang_2005,
	Author = {Q. Wang and Sanjeev R. Kulkarni and Sergio Verd\'{u}},
	Date-Added = {2006-12-13 12:17:47 -0800},
	Date-Modified = {2007-07-23 16:56:10 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {9},
	Pages = {3064-3074},
	Rating = {3},
	Read = {Yes},
	Title = {Divergence Estimation of Continuous Distributions based on Data-Dependent Partitions},
	Volume = {51},
	Year = {2005}}

@article{lugosi_1996_ann_sta,
	Author = {G. Lugosi and A. B. Nobel},
	Date-Added = {2006-12-12 11:35:00 -0800},
	Date-Modified = {2017-03-11 02:35:43 +0000},
	Journal = {The Annals of Statistics},
	Number = {2},
	Pages = {687-706},
	Rating = {5},
	Read = {Yes},
	Title = {Consistency of Data-Driven Histogram Methods for Density Estimation and Classification},
	Volume = {24},
	Year = {1996}}

@article{rabiner_1989,
	Author = {L. R. Rabiner},
	Date-Added = {2006-11-14 12:48:27 -0800},
	Date-Modified = {2006-11-14 12:50:09 -0800},
	Journal = {Proceedings of the IEEE},
	Month = {February},
	Number = {2},
	Pages = {257-286},
	Rating = {3},
	Read = {Yes},
	Title = {A tutorial on hidden {M}arkov models and selected applications in speech recognition},
	Volume = {77},
	Year = {1989}}

@conference{learned_1992,
	Author = {R. E. Learned and W.C. Karl and Alan S. Willsky},
	Booktitle = {Proc. IEEE Conf. Time Scale and Time Frequency Analysis},
	Date-Added = {2006-06-11 14:41:54 -0700},
	Date-Modified = {2006-06-11 14:44:50 -0700},
	Pages = {109-112},
	Rating = {1},
	Read = {Yes},
	Title = {Wavelet packet based transient signal classification},
	Year = {1992}}

@conference{fisher_2000,
	Author = {J. W. {Fisher III} and T. Darrel and W.T. Freeman and P. Viola},
	Booktitle = {Advances in Neural Information Processing System, Denver, USA},
	Date-Modified = {2006-08-29 16:52:10 -0700},
	Month = {November},
	Publisher = {Advances in Neural Information Processing Systems},
	Title = {Learning joint Statistical Models for Audio-Visual fusion and Segregation},
	Year = {2000}}

@conference{silva_2006,
	Author = {Jorge Silva and Shrikanth Narayanan},
	Booktitle = {IEEE International Symposium on Information Theory},
	Date-Modified = {2010-03-15 18:02:19 -0400},
	Month = {July},
	Title = {Upper Bound Kullback-Leibler Divergence for Hidden {M}arkov Models with Application as Discrimination Measure for Speech Recognition},
	Year = {2006}}

@book{michie_1994,
	Author = {D. Michie and D. J. Spiegelhalter and C.C. Taylor},
	Date-Added = {2006-10-13 17:22:52 -0700},
	Date-Modified = {2006-10-13 17:25:46 -0700},
	Publisher = {Hertfordshire, U.K.: Ellis Horwood},
	Title = {Machine Learning, Neural and Statistical Classification},
	Year = {1994}}

@article{laine_1993,
	Author = {A. Laine and Jian Fan},
	Date-Added = {2006-09-12 16:35:44 -0700},
	Date-Modified = {2006-09-12 16:37:32 -0700},
	Journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Number = {11},
	Pages = {1186-1191},
	Rating = {2},
	Read = {Yes},
	Title = {Texture Classification by Wavelet Packet Signatures},
	Volume = {15},
	Year = {1993}}

@article{chang_1993,
	Author = {T. Chang and C.C. Jay Kuo},
	Date-Added = {2006-09-12 16:31:59 -0700},
	Date-Modified = {2006-09-12 16:33:57 -0700},
	Journal = {IEEE Transactions on Image Processing},
	Number = {4},
	Pages = {429-441},
	Rating = {2},
	Read = {Yes},
	Title = {Texture Analysis and Classification with Tree-Structured Wavelet Transform},
	Volume = {2},
	Year = {1993}}

@article{soman_1993,
	Author = {A. K. Soman and P. P. Vaidyanathan},
	Date-Added = {2006-09-12 11:35:43 -0700},
	Date-Modified = {2006-09-12 11:37:57 -0700},
	Journal = {IEEE Transactions on Signal Processing},
	Number = {3},
	Pages = {1170-1183},
	Title = {On Orthonormal Wavelet and Paraunitary Filter Banks},
	Volume = {41},
	Year = {1993}}

@article{daubechies_1988,
	Author = {Ingrid Daubechies},
	Date-Added = {2006-09-12 11:26:00 -0700},
	Date-Modified = {2006-09-12 11:27:59 -0700},
	Journal = {Commun. on Pure and Appl. Math.},
	Pages = {909-996},
	Title = {Orthonormal bases of compactly supported wavelets},
	Volume = {41},
	Year = {1988}}

@article{silva_sub_2006,
	Author = {Jorge Silva and Shrikanth Narayanan},
	Date-Added = {2006-09-01 07:59:37 -0700},
	Date-Modified = {2006-10-01 15:41:05 -0700},
	Journal = {submitted for review.},
	Month = {September},
	Rating = {4},
	Read = {Yes},
	Title = {Minimum Probability of Error Signal Representation based on a Rate-Distortion Optimality Criterion},
	Year = {2006}}

@book{gray_2004,
	Author = {R. Gray and Lee D. Davisson},
	Date-Added = {2006-08-24 15:29:10 -0700},
	Date-Modified = {2006-08-24 15:30:24 -0700},
	Publisher = {Cambridge Univ Press},
	Title = {Introduction to Statistical Signal Processing},
	Year = {2004}}

@article{nobel_1997,
	Author = {Andrew B. Nobel},
	Date-Added = {2006-08-18 15:37:22 -0700},
	Date-Modified = {2006-08-18 15:39:21 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Month = {July},
	Number = {4},
	Pages = {1122-1133},
	Title = {Recursive Partitioning to Reduce Distortion},
	Volume = {43},
	Year = {1997}}

@article{vapnik_1971,
	Author = {Vladimir Vapnik and A. J. Chervonenkis},
	Date-Added = {2006-08-16 17:10:51 -0700},
	Date-Modified = {2008-01-10 15:31:22 -0800},
	Journal = {Theory of Probability Apl.},
	Pages = {264-280},
	Rating = {5},
	Read = {Yes},
	Title = {On the Uniform convergence of relative frequencies of events to their probabilities},
	Volume = {16},
	Year = {1971}}

@book{vapnik_1979,
	Author = {Vladimir Vapnik},
	Date-Added = {2006-08-16 17:03:29 -0700},
	Date-Modified = {2006-08-16 17:06:49 -0700},
	Publisher = {Springer - Verlag, New York},
	Title = {Estimation of dependencies based on empirical Data},
	Year = {1979}}

@inbook{bousquet_2004,
	Author = {Oliver Bousquet and S. Boucheron and G. Lugosi},
	Date-Added = {2006-08-16 11:57:28 -0700},
	Date-Modified = {2006-08-16 12:02:07 -0700},
	Publisher = {ESAIM: Probability and Statistics, URL:http:/www.emath.fr/ps},
	Title = {Theory of Classification: A Survey of Recent Advances},
	Year = {2004}}

@article{scott_2006,
	Author = {Clayton Scott and Robert D. Nowak},
	Date-Added = {2006-08-11 17:39:48 -0700},
	Date-Modified = {2006-08-11 17:42:18 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Month = {April},
	Number = {4},
	Pages = {1335-1353},
	Read = {Yes},
	Title = {Minimax-Optimal Classification with Dyadic Decision Trees},
	Volume = {52},
	Year = {2006}}

@book{quatieri_2002,
	Author = {Thomas F. Quatieri},
	Date-Added = {2006-08-10 18:40:06 -0700},
	Date-Modified = {2006-08-10 18:42:02 -0700},
	Publisher = {Prentice Hall},
	Title = {Discrete-time Speech Signal Processing principles and practice},
	Year = {2002}}

@book{vapnik_1999,
	Author = {Vladimir Vapnik},
	Date-Added = {2006-08-10 18:16:08 -0700},
	Date-Modified = {2006-08-10 18:17:58 -0700},
	Publisher = {Springer - Verlag, New York},
	Rating = {4},
	Read = {Yes},
	Title = {The Nature of Statistical Learning Theory},
	Year = {1999}}

@book{vapnik_1998,
	Author = {Vladimir Vapnik},
	Date-Added = {2006-08-10 18:12:38 -0700},
	Date-Modified = {2006-08-10 18:15:15 -0700},
	Publisher = {John Wiley},
	Rating = {4},
	Read = {Yes},
	Title = {Statistical Learning Theory},
	Year = {1998}}

@article{donoho_1998,
	Author = {David L. Donoho and Martin Vetterli and R. A. De{V}ore and Ingrid Daubechies},
	Date-Added = {2006-06-20 22:10:06 -0700},
	Date-Modified = {2006-06-20 22:13:00 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2435-2476},
	Rating = {4},
	Read = {Yes},
	Title = {Data Compression and Harmonic Analysis},
	Volume = {44},
	Year = {1998}}

@book{cormen_1990,
	Author = {T.H. Cormen and C.E. Leiserson and R. L. Rivest},
	Date-Added = {2006-06-14 22:15:02 -0700},
	Date-Modified = {2006-06-14 22:18:52 -0700},
	Publisher = {The MIT Press, Cambridge, Massachusetts},
	Title = {Introduction to Algorithms},
	Year = {1990}}

@article{yang_1992,
	Author = {X. Yang and K. Wang and S. A. Shamma},
	Date-Added = {2006-06-14 11:01:36 -0700},
	Date-Modified = {2006-06-14 11:04:22 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Month = {March},
	Number = {2},
	Pages = {824-839},
	Title = {Auditory Representation of Acoustic Signals},
	Volume = {38},
	Year = {1992}}

@article{willsky_2002,
	Author = {Alan S. Willsky},
	Date-Added = {2006-06-11 19:12:46 -0700},
	Date-Modified = {2006-06-11 19:15:09 -0700},
	Journal = {Proceedings of the IEEE},
	Month = {August},
	Number = {8},
	Pages = {1396-1458},
	Rating = {3},
	Read = {Yes},
	Title = {Multiresolution {M}arkov models for signal and image processing},
	Volume = {90},
	Year = {2002}}

@article{do_2002,
	Author = {M. N. Do and Martin Vetterli},
	Date-Added = {2006-06-11 19:09:53 -0700},
	Date-Modified = {2010-03-15 17:54:41 -0400},
	Journal = {IEEE Transactions on Image Processing},
	Number = {2},
	Pages = {146-158},
	Rating = {3},
	Read = {Yes},
	Title = {Wavelet-based texture retrieval using generalized gaussian densities and {K}ullback-{L}eibler distance},
	Volume = {11},
	Year = {2002}}

@article{crouse_1998,
	Author = {M. S. Crouse and Robert D. Nowak and R. G. Baraniuk},
	Date-Added = {2006-06-11 19:06:13 -0700},
	Date-Modified = {2006-06-11 19:09:05 -0700},
	Journal = {IEEE Transactions on Signal Processing},
	Month = {April},
	Number = {46},
	Pages = {886-902},
	Rating = {3},
	Read = {Yes},
	Title = {Wavelet-based statistical signal processing using hidden {M}arkov models},
	Volume = {46},
	Year = {1998}}

@article{saito_1994,
	Author = {N. Saito and R. R. Coifman},
	Date-Added = {2006-06-11 17:17:13 -0700},
	Date-Modified = {2010-03-15 17:57:08 -0400},
	Journal = {in Proc. SPIE 2303, Mathematical Imaging: Wavelet Applications in Signal and Image Processing},
	Pages = {2-14},
	Read = {Yes},
	Title = {Local Discriminant Basis},
	Year = {1994}}

@article{scott_2004,
	Author = {Clayton Scott and Robert D. Nowak},
	Date-Added = {2006-06-11 12:51:52 -0700},
	Date-Modified = {2006-06-11 12:54:12 -0700},
	Journal = {IEEE Transactions on Signal Processing},
	Month = {August},
	Number = {8},
	Pages = {2264-2274},
	Rating = {3},
	Read = {Yes},
	Title = {TEMPLAR: A Wavelet-Based framework for Pattern Learning and Analysis},
	Volume = {52},
	Year = {2004}}

@article{goyal_2001,
	Author = {V. K Goyal},
	Date-Added = {2006-06-11 11:31:28 -0700},
	Date-Modified = {2006-06-11 11:34:02 -0700},
	Journal = {IEEE Signal Processing Magazine},
	Month = {September},
	Pages = {9-21},
	Rating = {3},
	Read = {Yes},
	Title = {Theoretical Foundation of Transform Coding},
	Year = {2001}}

@book{varadhan_2001,
	Author = {S.R.S. Varadhan},
	Date-Added = {2006-05-29 15:27:51 -0700},
	Date-Modified = {2006-05-29 15:29:40 -0700},
	Publisher = {American Mathematical Society},
	Rating = {5},
	Read = {Yes},
	Title = {Probability Theory},
	Year = {2001}}

@article{darbellay_1999,
	Author = {Georges A. Darbellay and Igor Vajda},
	Date-Added = {2006-05-26 12:56:42 -0700},
	Date-Modified = {2006-05-26 12:59:20 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {4},
	Pages = {1315-1321},
	Rating = {3},
	Read = {Yes},
	Title = {Estimation of the Information by an Adaptive partition of the observation space},
	Volume = {45},
	Year = {1999}}

@book{breiman_1968,
	Author = {Leo Breiman},
	Date-Added = {2006-05-18 14:06:20 -0700},
	Date-Modified = {2006-05-18 14:09:01 -0700},
	Publisher = {Addison-Wesley},
	Title = {Probability},
	Year = {1968}}

@article{kumar_2001,
	Author = {S. Kumar and J. Ghosh and M. M. Crawford},
	Date-Added = {2006-05-14 09:05:37 -0700},
	Date-Modified = {2006-05-14 09:08:33 -0700},
	Journal = {IEEE Transactions on Geoscience and Remote Sensing},
	Month = {July},
	Number = {7},
	Pages = {1368-1379},
	Rating = {2},
	Read = {Yes},
	Title = {Best-Bases Feature Extraction Algorithms for Classification of Hyperspectral Data},
	Volume = {39},
	Year = {2001}}

@article{etemad_1998,
	Author = {Kamran Etemad and Rama Chellapa},
	Date-Added = {2006-05-14 08:52:31 -0700},
	Date-Modified = {2006-05-14 09:17:53 -0700},
	Journal = {IEEE Transactions on Image Processing},
	Month = {October},
	Number = {10},
	Pages = {1453-1465},
	Rating = {2},
	Read = {Yes},
	Title = {Separability-Based Multiscale Basis Selection and Feature Extraction for Signal and Image Classification},
	Volume = {7},
	Year = {1998}}

@article{cover_1977,
	Author = {T. M. Cover and J. M. Van~Campenhout},
	Date-Added = {2006-05-12 12:07:09 -0700},
	Date-Modified = {2006-05-12 12:40:44 -0700},
	Journal = {IEEE Transactions on Systems, Man. Cybern.},
	Pages = {657-661},
	Title = {On the possible ordering in the measurement selection problem},
	Volume = {7},
	Year = {1977}}

@article{novovicova_1996,
	Author = {Jana Novovicova and Pavel Pudil and Josef Kittler},
	Date-Added = {2006-05-12 11:48:09 -0700},
	Date-Modified = {2010-03-15 17:56:29 -0400},
	Journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Number = {2},
	Pages = {218-223},
	Title = {Divergence Based Feature Selection for Multimodal Class Densities},
	Volume = {18},
	Year = {1996}}

@article{trunk_1979,
	Author = {G.V. Trunk},
	Date-Added = {2006-05-10 21:46:08 -0700},
	Date-Modified = {2006-05-14 08:58:01 -0700},
	Journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Pages = {306-307},
	Title = {A problem of dimensionality: A simple example},
	Volume = {1},
	Year = {1979}}

@article{gray_1998_b,
	Author = {R.M. Gray and D.L. Neuhoff},
	Date-Added = {2006-05-04 22:52:17 -0700},
	Date-Modified = {2006-05-04 22:54:28 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Month = {October},
	Pages = {2325-2384},
	Read = {Yes},
	Title = {Quantization},
	Volume = {44},
	Year = {1998}}

@book{wozencraft_1965,
	Author = {J.M. Wozencraft and I.M. Jacobs},
	Date-Added = {2006-05-04 22:33:03 -0700},
	Date-Modified = {2006-05-04 22:34:51 -0700},
	Publisher = {Waveland Press},
	Rating = {5},
	Read = {Yes},
	Title = {Principles of Communication Engineering},
	Year = {1965}}

@article{coifman_1992,
	Author = {R. R. Coifman and M. V. Wickerhauser},
	Date-Added = {2006-05-04 20:02:12 -0700},
	Date-Modified = {2006-12-08 19:21:28 -0800},
	Journal = {IEEE Transactions on Information Theory},
	Month = {March},
	Number = {2},
	Pages = {713-718},
	Read = {Yes},
	Title = {Entropy-based algorithm for best basis selection},
	Volume = {38},
	Year = {1992}}

@article{wipf_2004,
	Author = {D. P. Wipf and B. D. Rao},
	Date-Added = {2006-05-04 20:00:00 -0700},
	Date-Modified = {2006-05-04 20:01:03 -0700},
	Journal = {IEEE Transactions on Signal Processing},
	Month = {August},
	Number = {8},
	Read = {Yes},
	Title = {Sparse Bayesian learning for basis selection},
	Volume = {52},
	Year = {2004}}

@article{rao_1999,
	Author = {B. D. Rao and K. K. Kreutz-Delgado},
	Date-Added = {2006-05-04 19:57:53 -0700},
	Date-Modified = {2006-05-04 19:59:17 -0700},
	Journal = {IEEE Transactions on Signal Processing},
	Month = {January},
	Number = {1},
	Title = {An affine scaling methodology for best basis selection},
	Volume = {47},
	Year = {1999}}

@article{beheshti_2005,
	Author = {S. Beheshti and M. A. Dahleh},
	Date-Added = {2006-05-04 19:54:12 -0700},
	Date-Modified = {2006-05-04 19:55:32 -0700},
	Journal = {IEEE Transactions on Signal Processing},
	Month = {October},
	Number = {10},
	Title = {A new information-theoretic approach to signal denoising and best basis selection},
	Volume = {53},
	Year = {2005}}

@article{cohen_2002,
	Author = {A. Cohen and I. Daubechies and O. Guleryuz and M. Orchard},
	Date-Added = {2006-05-04 19:49:52 -0700},
	Date-Modified = {2006-05-14 09:01:01 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Month = {July},
	Number = {1},
	Rating = {3},
	Read = {Yes},
	Title = {On the importance of combining Wavelet-Based nonlinear approximation with coding strategies},
	Volume = {48},
	Year = {2002}}

@article{ramchandran_1996,
	Author = {K. Ramchandran and M. Vetterli and C. Herley},
	Date-Added = {2006-05-04 19:46:36 -0700},
	Date-Modified = {2006-06-11 12:24:07 -0700},
	Journal = {Proceedings of the IEEE},
	Month = {April},
	Number = {4},
	Pages = {541-560},
	Rating = {3},
	Read = {Yes},
	Title = {Wavelet, subband coding, and best bases},
	Volume = {84},
	Year = {1996}}

@article{lozano_2003,
	Author = {B. Beferull-Lozano and A. Ortega},
	Date-Added = {2006-05-04 19:43:49 -0700},
	Date-Modified = {2006-05-14 08:59:25 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Month = {January},
	Number = {1},
	Pages = {129-150},
	Rating = {4},
	Read = {Yes},
	Title = {Efficient Quantization for Overcomplete Expansions in $\mathbb{R}^N$},
	Volume = {49},
	Year = {2003}}

@article{cvetkovic_2001,
	Author = {Z. Cvetkovic and M. Vetterli},
	Date-Added = {2006-05-04 19:41:59 -0700},
	Date-Modified = {2006-05-14 09:00:49 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Month = {January},
	Number = {1},
	Pages = {59-73},
	Title = {On simple oversampled A/D conversion in L2(R)},
	Volume = {47},
	Year = {2001}}

@article{goyal_1998,
	Author = {V. K Goyal and M. Vetterli and N. T. Thao},
	Date-Added = {2006-05-04 19:38:42 -0700},
	Date-Modified = {2006-05-14 08:57:46 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {7},
	Pages = {16-31},
	Read = {Yes},
	Title = {Quantized Overcomplete Expansions in $\mathbb{R}^N$: Analysis, Synthesis and Algorithms},
	Volume = {44},
	Year = {1998}}

@article{witsenhausen_1980,
	Author = {Hans S. Witsenhausen},
	Date-Added = {2006-05-03 18:50:13 -0700},
	Date-Modified = {2006-05-14 09:00:10 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Pages = {518-521},
	Title = {Indirect Rate Distortion Problems},
	Volume = {it-36},
	Year = {1980}}

@article{wolf_1970,
	Author = {Jack K. Wolf and Jacob Ziv},
	Date-Added = {2006-05-03 18:46:55 -0700},
	Date-Modified = {2006-05-14 09:04:37 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {4},
	Pages = {406-411},
	Title = {Transmission of Noisy Information to a Noisy Receiver with Minimum Distortion},
	Volume = {it-16},
	Year = {1970}}

@book{ripley_1996,
	Author = {B. D. Ripley},
	Date-Added = {2006-04-06 14:42:41 -0700},
	Date-Modified = {2006-04-06 14:44:34 -0700},
	Publisher = {Cambridge Univ Press},
	Title = {Patten Recognition and Neural Networks},
	Year = {1996}}

@article{nobel_2002,
	Author = {Andrew B. Nobel},
	Date-Added = {2006-03-22 10:10:54 -0800},
	Date-Modified = {2006-05-14 08:58:44 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {8},
	Pages = {2362-2368},
	Rating = {3},
	Read = {Yes},
	Title = {Analysis of a Complexity-Based Pruning Scheme for Classification Tree},
	Volume = {48},
	Year = {2002}}

@book{halmos_1950,
	Author = {P. R. Halmos},
	Date-Added = {2006-03-14 10:52:44 -0800},
	Date-Modified = {2006-03-14 11:05:50 -0800},
	Publisher = {Van Nostrand, New York},
	Title = {Measure Theory},
	Year = {1950}}

@phdthesis{vasconcelos_2000,
	Author = {Nuno Vasconcelos},
	Date-Added = {2006-03-13 20:21:29 -0800},
	Date-Modified = {2006-03-13 20:23:30 -0800},
	School = {Mass. Inst. of Technol.},
	Title = {Bayesian Model for visual Information Retrieval},
	Year = {2000}}

@article{ephraim_1998,
	Author = {Yariv Ephraim and Robert M. Gray},
	Date-Added = {2006-03-07 10:47:28 -0800},
	Date-Modified = {2006-05-14 08:58:25 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {4},
	Pages = {826-834},
	Rating = {3},
	Title = {A Unified approach for Encoding Clean and Noise Sources by Means of Waveform and Autoregressive Model Vector Quantization},
	Volume = {34},
	Year = {1998}}

@article{shannon_1959,
	Author = {C. E. Shannon},
	Date-Added = {2006-03-07 09:36:05 -0800},
	Date-Modified = {2006-03-07 09:38:17 -0800},
	Journal = {in IRE Conv. Rec.},
	Number = {142-163},
	Rating = {5},
	Title = {Coding Theorems for a discrete source with fidelity criterion},
	Volume = {7},
	Year = {1959}}

@article{berger_1998,
	Author = {Toby Berger and Jerry D. Gibson},
	Date-Added = {2006-03-07 09:32:10 -0800},
	Date-Modified = {2006-05-14 09:00:22 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2693-2723},
	Rating = {5},
	Title = {Lossy Source Coding},
	Volume = {44},
	Year = {1998}}

@book{gray_1990,
	Author = {R.M. Gray},
	Date-Added = {2006-03-07 09:30:33 -0800},
	Date-Modified = {2006-03-07 09:31:38 -0800},
	Publisher = {Norwell, MA: Kluwer Academic},
	Title = {Source Coding Theory},
	Year = {1990}}

@book{gersho_1992,
	Author = {A. Gersho and R.M. Gray},
	Date-Added = {2006-03-07 09:27:55 -0800},
	Date-Modified = {2006-03-07 09:29:59 -0800},
	Publisher = {Norwell, MA: Kluwer Academic},
	Title = {Vector Quantization and Signal Compression},
	Year = {1992}}

@article{amuallim_1996,
	Author = {H. Amuallim},
	Date-Added = {2006-02-18 16:17:27 -0800},
	Date-Modified = {2006-08-29 16:53:51 -0700},
	Journal = {Artificial Intelligence},
	Pages = {347-362},
	Title = {An efficient algorithm for optimal pruning of decision trees},
	Volume = {83},
	Year = {1996}}

@article{bohanec_1994,
	Author = {M. Bohanec and I. Bratko},
	Date-Added = {2006-02-18 16:12:34 -0800},
	Date-Modified = {2006-02-18 16:15:13 -0800},
	Journal = {Machine Learning},
	Pages = {223-250},
	Title = {Trading Accuracy for simplicity in Decision Trees},
	Volume = {15},
	Year = {1994}}

@article{daubechies_1990,
	Author = {Ingrid Daubechies},
	Date-Added = {2006-02-08 16:54:15 -0800},
	Date-Modified = {2006-05-14 09:04:21 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Pages = {961-1005},
	Title = {The Wavelet transform, time-frequency localization and signal analysis},
	Volume = {36},
	Year = {1990}}

@article{chou_1989,
	Author = {P. Chou and T. Lookabaugh and R. Gray},
	Date-Added = {2006-02-07 17:57:54 -0800},
	Date-Modified = {2006-08-29 16:51:38 -0700},
	Journal = {IEEE Transactions on Information Theory},
	Number = {2},
	Pages = {299-315},
	Rating = {3},
	Read = {Yes},
	Title = {Optimal pruning with applications to tree-structure source coding and modeling},
	Volume = {35},
	Year = {1989}}

@article{scott_2005,
	Annote = {Describe the problem of general family pruning with sized based penalties
		and particular results for the case of subadditive penalties},
	Author = {Clayton Scott},
	Date-Added = {2006-02-07 17:54:08 -0800},
	Date-Modified = {2006-02-07 17:56:18 -0800},
	Journal = {IEEE Transactions on Signal Processing},
	Number = {12},
	Pages = {4518-4525},
	Rating = {4},
	Read = {Yes},
	Title = {Tree Pruning with Subadditive Penalties},
	Volume = {53},
	Year = {2005}}

@book{breiman_1984,
	Author = {Leo Breiman and J. Friedman and R. Olshen and C. Stone},
	Date-Added = {2006-02-07 17:51:04 -0800},
	Date-Modified = {2006-06-28 23:24:41 -0700},
	Publisher = {Belmont, CA: Wadsworth},
	Rating = {4},
	Title = {Classification and Regression Trees},
	Year = {1984}}

@article{mallat_1989,
	Author = {S. Mallat},
	Date-Added = {2006-02-06 17:54:35 -0800},
	Date-Modified = {2006-08-11 17:32:47 -0700},
	Journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Month = {July},
	Pages = {674-693},
	Title = {A Theory for Multiresolution Signal Decomposition: the Wavelet representation},
	Volume = {11},
	Year = {1989}}

@book{daubechies_1992,
	Author = {Ingrid Daubechies},
	Date-Added = {2006-02-06 17:41:23 -0800},
	Date-Modified = {2006-02-06 17:42:35 -0800},
	Publisher = {Philadelphia: SIAM},
	Title = {Ten Lectures on Wavelets},
	Year = {1992}}

@article{mintzer_1985,
	Author = {F. Mintzer},
	Date-Added = {2006-02-06 17:31:37 -0800},
	Date-Modified = {2006-02-06 17:34:18 -0800},
	Journal = {IEEE Transactions on Acoustic, Speech and Signal Processing},
	Month = {June},
	Pages = {626-630},
	Title = {Filters for distortion-free two-band multirate filter banks},
	Volume = {ASSP-33},
	Year = {1985}}

@book{vaidyanathan_1993,
	Author = {P. P. Vaidyanathan},
	Date-Added = {2006-02-06 17:27:56 -0800},
	Date-Modified = {2006-02-06 17:30:12 -0800},
	Publisher = {Englewood Cliffs:NY Prentice-Hall},
	Title = {Multirate Systems and Filter Banks},
	Year = {1993}}

@book{vetterli_1995,
	Author = {Martin Vetterli and Jelena Kovacevic},
	Date-Added = {2006-02-06 17:23:07 -0800},
	Date-Modified = {2006-02-06 17:25:54 -0800},
	Publisher = {Englewood Cliffs, NY: Prentice-Hall},
	Title = {Wavelet and Subband Coding},
	Year = {1995}}

@techreport{coffman1990,
	Author = {R. Coifman and Y. Meyer and S. Quake and V. Wickerhauser},
	Date-Added = {2006-02-02 17:01:36 -0800},
	Date-Modified = {2006-02-06 17:50:07 -0800},
	Institution = {Numerical Algorithms Research Group, New Haven, CT, Yale University},
	Title = {Signal processing and compression with wavelet packets},
	Year = {1990}}

@article{ramchandran1993,
	Author = {K. Ramchandran and Martin Vetterli},
	Date-Added = {2006-02-02 16:44:30 -0800},
	Date-Modified = {2006-05-14 08:58:59 -0700},
	Journal = {IEEE Transactions on Image Processing},
	Number = {2},
	Pages = {160-175},
	Title = {Best Wavelet Packet Bases in Rate-Distortion Sense},
	Volume = {2},
	Year = {1993}}

@book{kullback1958,
	Author = {S. Kullback},
	Date-Added = {2006-01-28 15:29:49 -0800},
	Date-Modified = {2006-01-28 15:31:16 -0800},
	Publisher = {New York: Wiley},
	Read = {Yes},
	Title = {Information theory and Statistics},
	Year = {1958}}

@article{raudys1991,
	Author = {S. J. Raudys and A. K. Jain},
	Date-Added = {2006-01-19 13:17:37 -0800},
	Date-Modified = {2006-05-14 09:03:55 -0700},
	Journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Month = {March},
	Pages = {252-264},
	Title = {Small sample size effects in statistical Pattern Recognition},
	Volume = {13},
	Year = {1991}}

@book{duda1983,
	Author = {R. O. Duda and P. E. Hart},
	Date-Added = {2006-01-19 13:12:45 -0800},
	Date-Modified = {2006-01-19 13:14:48 -0800},
	Publisher = {New York: Wiley},
	Title = {Pattern Classification and Scene Analysis},
	Year = {1983}}

@article{jain2000,
	Author = {A. K. Jain and R. P. W. Duin and J. Mao},
	Date-Added = {2006-01-19 13:08:15 -0800},
	Date-Modified = {2006-05-14 09:04:09 -0700},
	Journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Month = {April},
	Pages = {4-36},
	Title = {Statistical pattern recognition: A review},
	Volume = {22},
	Year = {2000}}

@article{hughes1968,
	Author = {G. F. Hughes},
	Date-Added = {2006-01-19 12:40:48 -0800},
	Date-Modified = {2006-01-19 13:06:34 -0800},
	Journal = {IEEE Transactions on Information Theory},
	Month = {January},
	Number = {1},
	Pages = {55-63},
	Title = {On the mean accuracy of statistical pattern recognition},
	Volume = {IT-14},
	Year = {1968}}

@book{devroye1996,
	Author = {L. Devroye and L. Gy{\"o}rfi and G. Lugosi},
	Date-Added = {2006-01-19 09:53:33 -0800},
	Date-Modified = {2010-03-15 10:38:40 -0400},
	Publisher = {New York: Springer-Verlag},
	Title = {A Probabilistic Theory of Pattern Recognition},
	Year = {1996}}

@article{jimenez1999,
	Author = {Luis O. Jimenez and David A. Landgrebe},
	Date-Added = {2005-12-31 10:52:36 -0800},
	Date-Modified = {2005-12-31 10:57:28 -0800},
	Journal = {IEEE Transactions on Geoscience and Remote Sensing},
	Month = {November},
	Number = {6},
	Pages = {2653-2667},
	Title = {Hyperspectral Data Analysis and Supervised Feature Reduction via Projection Pursuit},
	Volume = {37},
	Year = {1999}}

@article{schmid2001,
	Author = {Natalia A. Schmid and Joseph A. O'Sullivan},
	Date-Added = {2005-12-31 10:47:31 -0800},
	Date-Modified = {2006-01-19 10:35:32 -0800},
	Journal = {IEEE Transactions on Information Theory},
	Month = {November},
	Number = {7},
	Pages = {2903-2920},
	Rating = {2},
	Title = {Thresholding Method for Dimensionality Reduction in Recognition System},
	Volume = {47},
	Year = {2001}}

@article{vasconcelos2004,
	Author = {Nuno Vasconcelos},
	Booktitle = {IEEE Transaction on Signal Processing},
	Date-Added = {2005-12-31 10:38:42 -0800},
	Date-Modified = {2010-03-15 17:58:00 -0400},
	Journal = {IEEE Transactions on Signal Processing},
	Number = {8},
	Pages = {2322-2336},
	Rating = {5},
	Read = {Yes},
	Title = {Minimum Probability of Error Image Retrieval},
	Volume = {52},
	Year = {2004}}

@book{gray_1990_b,
	Author = {R. M. Gray},
	Publisher = {Springer - Verlag, New York},
	Title = {Entropy and Information Theory},
	Year = {1990}}

@article{padmanabhan_2005,
	Author = {M. Padmanabhan and S. Dharanipragada},
	Date-Modified = {2006-05-14 09:00:32 -0700},
	Journal = {IEEE Transactions on Speech and Audio Processing},
	Month = {July},
	Number = {4},
	Pages = {512-519},
	Title = {Maximizing information content in feature extraction},
	Volume = {13},
	Year = {2005}}

@article{fisher_2002,
	Author = {John W. {Fisher III} and Martin Wainwright and Erik Sudderth and Alan S. Willsky},
	Date-Modified = {2006-08-17 16:46:58 -0700},
	Journal = {International Journal of High Performance Computing Applications},
	Title = {Statistical and Information-Theoretic Methods For Self-Organization And Fusion Of Multimodal, Networked},
	Year = {2002}}

@article{butz_2005,
	Author = {T. Butz and J.-Ph. Thiran},
	Journal = {Elsevier Signal Processing},
	Pages = {875-902},
	Title = {From error probability to information theoretic (multi-modal) signal processing},
	Volume = {85},
	Year = {2005}}

@article{shannon_1948,
	Author = {C. E. Shannon},
	Date-Modified = {2010-03-19 11:09:21 -0400},
	Journal = {Bell System Tech, J.},
	Pages = {379-423; 623-656},
	Title = {A mathematical theory of communication},
	Volume = {27},
	Year = {1948}}

@inproceedings{costa_2005,
	Author = {J.A. Costa and A.O. Hero},
	Organization = {Proceedings of IEEE ICAASP},
	Title = {Classifcation Constrained Dimensionality Reduction},
	Year = {2005}}

@inbook{fukunaga_1990,
	Author = {K. Fukunaga},
	Publisher = {Academic Press},
	Title = {Introduction to Statistical Pattern Recognition},
	Year = {1990}}

